Solving connectivity problems parameterized by treewidth in single exponential time

For the vast majority of local graph problems standard dynamic programming techniques give c^tw V^O(1) algorithms, where tw is the treewidth of the input graph. On the other hand, for problems with a global requirement (usually connectivity) the best-known algorithms were naive dynamic programming schemes running in tw^O(tw) V^O(1) time. We breach this gap by introducing a technique we dubbed Cut&Count that allows to produce c^tw V^O(1) Monte Carlo algorithms for most connectivity-type problems, including Hamiltonian Path, Feedback Vertex Set and Connected Dominating Set, consequently answering the question raised by Lokshtanov, Marx and Saurabh [SODA'11] in a surprising way. We also show that (under reasonable complexity assumptions) the gap cannot be breached for some problems for which Cut&Count does not work, like CYCLE PACKING. The constant c we obtain is in all cases small (at most 4 for undirected problems and at most 6 for directed ones), and in several cases we are able to show that improving those constants would cause the Strong Exponential Time Hypothesis to fail. Our results have numerous consequences in various fields, like FPT algorithms, exact and approximate algorithms on planar and H-minor-free graphs and algorithms on graphs of bounded degree. In all these fields we are able to improve the best-known results for some problems.

==> negatives-seth-steiner.tex <==
\renewcommand{\numcopies}{\ensuremath{m(5\blocksize n'+1)}\xspace}
\renewcommand{\numcopiessmall}{\ensuremath{5\blocksize n'+1}\xspace}

\subsection{\steinertree}
  
For the sake of simplicity we start with a proof for the weighted version of the \steinertree problem
and next reduce the weighted version to the unweighted one.

\defproblemu{\weightedst}{An undirected graph $G = (V,E)$ together with a weight function $c:E \rightarrow \Z_+$
, a set of terminals $\terms \subseteq V$ and an integer $\goalsize$}{Does there exist a tree in $G$ that contains all terminals $\terms$
  and the sum of its edges is at most $\goalsize$?}

\begin{theorem}\label{thm:wst-lower}
Assuming SETH, there cannot exist a constant $\eps>0$ and an algorithm that given an instance $(G=(V,E), c, \terms)$ with weights not exceeding $|V|^4$ together with a path decomposition of the graph $G$ of width $p$ solves the \weightedst problem in $(3-\eps)^p |V|^{O(1)}$ time.
\end{theorem}

\paragraph{Construction}

Given $\eps > 0$ and an instance $\Phi$ of SAT with $n$ variables and $m$ clauses we construct a graph $G$ as follows.
We first choose a constant integer $\blocksize$, which value depends on $\eps$ only.
The exact formula for $\blocksize$ is presented later.
We partition variables of $\Phi$ into groups $F_1,\ldots,F_{n'}$, each of size at most $\blockvars = \lfloor \log 3^\blocksize \rfloor$,
hence $n'=\lceil n/\blockvars \rceil$.
Note that now $\blocksize n' \sim n/\log 3$, the pathwidth of $G$ will be roughly $\blocksize n'$.
By $N$ let us denote the total number of vertices of the graph $G$ after the construction process.
We use $N$ only to set weights to edges, in fact, we use only weights $\{1,N,N^2,N^3,N^4\}$.

First, we add to the graph $G$ a vertex $r$, called a {\em root}, which is added to the set of terminals $\terms$.

We start with the description of a group gadget $\groupg$, which will enable us to encode $2^\blockvars$ possible assignments of one group of $\blockvars$ variables.
We create an independent set $V_\groupg$ of $3\blocksize$ vertices denoted as $v_\iv^\ivup$, where $1 \le \iv \le \blocksize$ and $1 \le \ivup \le 3$.
Let us denote $V_{\groupg,\iv} = \{v_\iv^1, v_\iv^2, v_\iv^3\}$.
To each set $V_{\groupg,\iv}$ we attach three guards $g_\iv^1,g_\iv^2,g_\iv^3$ which we add to the set of terminals $\terms$.
Those guards are used to ensure that each tree spanning all the terminals in $G$
contains at least two vertices out of each set $V_{\groupg,\iv}$, thus
we add the following edges of weight $N^2$: $\{g_\iv^1v_\iv^1, g_\iv^1v_\iv^2, g_\iv^2v_\iv^1, g_\iv^2v_\iv^3, g_\iv^3v_\iv^2, g_\iv^3v_\iv^3\}$.
Moreover for each $V_{\groupg,\iv}$ we add to the graph $G$ two vertices $h_\iv^1$,$h_\iv^2$ where $h_\iv^\ivup$ is 
connected with $v_\iv^\ivup$ and $v_\iv^{\ivup+1}$ by edges of weight $N$.
Furthermore for each $h_\iv^\ivup$ we add an edge $rh_\iv^\ivup$ of weight $1$.

In order to encode $2^\blockvars$ assignments we consider subsets of $V_\groupg$ that contain {\em exactly one}
vertex out of each set $V_{\groupg,\iv}$.
For a sequence $S=(s_1,\ldots,s_\blocksize) \in \{1,2,3\}^\blocksize$ by $S(V_\groupg)$ we denote
the set $\{v_\iv^{s_\iv} : 1 \le \iv \le \blocksize, v_\iv^{s_\iv} \in V_\groupg\}$.
For each sequence $S \in \{1,2,3\}^\blocksize$ we add two adjacent vertices $x_S,x_S'$,
where $x_S$ is also adjacent to all the vertices of $S(V_\groupg)$
(recall that $\blocksize$ and $\blockvars$ are constants depending only on $\eps$).
The weight of the edge $x_Sx_S'$ is $1$, whereas the weight of each edge between $x_S$ and $S(V_\groupg)$ is $N^3$.
Additionally we connect each vertex $x_S'$ with the root $r$ by an edge of weight $N^3$.
We add all the vertices $x_S$ to the set of terminals $\terms$.
A group gadget for $\blocksize=3$ is shown in Figure~\ref{fig:st}.

\begin{figure}
\begin{center}
\includegraphics{figures/fig-st.pdf}
\caption{Group gadget $\groupg$ for $\blocksize=3$. Only a few edge weights are given in the figure for readability. Dashed edges are connecting a vertex with the root $r$. 
  Terminal vertices are presented as squares.  }
\label{fig:st}
\end{center}
\end{figure}

Let $a_1 = \numcopies$.
For each group of variables $F_\iF$ we create $a_1$
copies of the group gadget $\groupg$ and denote them by $\groupg_\iF^\iB$ for $1 \le \iB \le a_1$.
For every fixed $\iF \le n'$ we connect the gadgets $\groupg_\iF^1, \groupg_\iF^2, \ldots, \groupg_\iF^{a_1}$
in a path-like manner using additional vertices.
More precisely, for each $\iB < a_1$ and every $\iv \le \blocksize$ we add two vertices $p_{\iv}^{\iF,\iB}$ and $q_{\iv}^{\iF,\iB}$.
Both of them are connected to the vertex $v_{\iv}^3$ of the gadget $\groupg_\iF^\iB$
and $v_{\iv}^1$ of the gadget $\groupg_\iF^{\iB+1}$,
however the two edges incident with the vertex $p_{\iv}^{\iF,\iB}$ are of weight $N^2$ whereas 
the two edges incident with the vertex $q_{\iv}^{\iF,\iB}$ are of weight $N$.
Additionally add an edge $rq_{\iv}^{\iF,\iB}$ of length $1$ and put $p_{\iv}^{\iF,\iB}$ to the set of terminals.
Furthermore for each $\iv \le \blocksize$ we connect the vertex $v_{\iv}^1$ of the gadget $\groupg_\iF^1$
with the root $r$ by an edge of weight $N$.
Moreover for each $\iv \le \blocksize$ we add
a vertex $w_{\iF,\iv}$ and connect it with the root $r$ by an edge of length $1$
and also connect it with the vertex $v_{\iv}^3$ of the gadget $\groupg_\iF^{a_1}$ 
by an edge of weight $N$.
By $\cG$ let us denote the set of all guard vertices $g_\iv^\ivup$ from all group gadgets in the whole graph $G$.
Similarly by $\cH,\cP,\cQ, \cW$ we denote sets of all vertices $h_\iv^\ivup,p_{\iv}^{\iF,\iB},q_{\iv}^{\iF,\iB},w_{\iF,\iv}$ 
in the whole graph $G$.

We have finished the part of the construction needed to encode an assignment and now we add vertices used
to check the satisfiability of the formula $\Phi$.
Observe that for a group of variables $F_\iF$ there are at most $2^{\blockvars}$ possible assignments
and there are $3^\blocksize \ge 2^{\blockvars}$ vertices $x_S$ for sequences $S$ from the set $\{1,2,3\}^\blocksize$ in each group gadget,
hence we can assign a {\em unique} sequence $S$ to each assignment.
Let $C_1,\ldots,C_m$ be the clauses of the formula $\Phi$.
For each clause $C_\iC$ we create $\numcopiessmall$ terminal vertices $c_\iC^{\ib}$, one for each $0 \le \ib < \numcopiessmall$.
The vertex $c_\iC^{\ib}$ can only be connected to gadgets $\groupg_\iF^{m\ib+\iC}$ for $1 \le \iF \le n'$.
For each group of variables $F_\iF$ we consider all sequences $S \in \{1,2,3\}^\blocksize$ that correspond 
to an assignment of $F_\iF$ satisfying the clause $C_\iC$.
For each such sequence $S$ and for each $0 \le \ib < \numcopiessmall$ we connect the vertex $x_S'$ from the gadget $\groupg_\iF^{m\ib+\iC}$
with the vertex $c_\iC^{\ib}$ by an edge of weight $N^4$.

We can view the whole construction as a matrix of group gadgets, where each row corresponds to some group of variables $F_\iF$
and each column is devoted to some clause in such a way that each clause gets $\numcopiessmall$ private columns (but not consecutive)
of the group gadget matrix as in Figure~\ref{fig:stmatrix}.

\begin{figure}[htbp]
\begin{center}
\includegraphics{figures/fig-stmatrix.pdf}
\caption{Gray rectangles represent group gadgets. Terminal vertices are presented as squares. Dashed edges connect have
  the root vertex $r$ as one of the endpoints. 
}
\label{fig:stmatrix}
\end{center}
\end{figure}

Let
$$\goalsize = a_1 \cdot N^4 + a_2 \cdot N^3 + a_3 \cdot N^2 + a_4 \cdot N + a_5 + a_6,$$
where
\begin{align*}
a_1 &= \numcopies, \\
a_2 &= 3^\blocksize n' a_1 = 3^\blocksize n' \numcopies, \\
a_3 &= \blocksize n' \cdot (4a_1-1) = \blocksize n' \cdot (4\numcopies - 1), \\
a_4 &= 2\blocksize n' a_1 = 2\blocksize n' \numcopies, \\
a_5 &= \blocksize n'a_1 = \blocksize n' \numcopies, \\
a_6 &= n'a_1 = n'\numcopies.
\end{align*}

\paragraph{Correctness}

\begin{lemma}\label{lem:lowerst1}
If $\Phi$ has a satisfying assignment, then there exists a tree spanning all terminals with the sum of weights equal to $\goalsize$.
\end{lemma}

\begin{proof}
Given a satisfying assignment $\phi$ of the formula $\Phi$ we construct a set of edges $E_0 \subseteq E(G)$ that spans all terminals.
Initially $E_0$ is empty and 
we start by describing which vertices from sets $V_\groupg$ of group gadgets will have an incident edge in the set $E_0$.
For each group of variables $F_\iF$ we consider the sequence $S \in \{1,2,3\}^\blocksize$ which corresponds to the restriction 
of the assignment $\phi$ to the variables of $F_\iF$.
Let
$$V_{\iF,\iv} = \bigcup_{\iB=1}^{a_1} (V_{\groupg_\iF^\iB,\iv} \setminus S(V_{\groupg_\iF^\iB})).$$
All the vertices from the set $V_{\iF,\iv}$ will have an incident edge in the set $E_0$.
Let $S=(s_1,\ldots,s_\blocksize)$.
For each $1 \le \iv \le \blocksize$ consider two cases.
\begin{itemize}
\item If $s_\iv=3$ (resp. $s_\iv=1$) then 
for each group gadget $\groupg_\iF^\iB$ for $1 \le \iB \le a_1$ we add three edges incident
with the vertex $h_{\iv}^1$ (resp. $h_{\iv}^2$) 
of total weight $2N+1$ to the set $E_0$.
In this way we connect the vertices $v_{\iv}^1,v_{\iv}^2$ (resp. $v_{\iv}^2,v_{\iv}^3$) to the root $r$.
\item If $s_{\iv}=2$ then for each $1 \le \iB < a_1$
we add three edges incident with the vertex $q_{\iv}^{\iF,\iB}$ of total weight $2N+1$ to the set $E_0$.
In this way we connect almost all the vertices $v_{\iv}^1,v_{\iv}^3$ to the root $r$
and the only vertices of the set $V_{\iF,\iv}$ that are not connected to the root are $v_{\iv}^1$ 
from the gadget $\groupg_\iF^1$ and $v_{\iv}^3$ from the gadget $\groupg_\iF^{a_1}$.
To connect the lacking vertex $v_{\iv}^1$ we use the edge that goes directly to the root (of weight $N$),
whereas for $v_{\iv}^3$ we use two edges incident with $w_{\iF,\iv}$ of weight $N$ and $1$.
\end{itemize}
Summing over all $\iF$ and $\iv$ weights of all edges used so far to connect vertices $V_{\iF,\iv}$ to the root equals $a_4\cdot N+a_5$.
Now for each guard $g \in \cG$ and for each vertex $p \in \cP$
we know that there exists at least one neighbour that is in some set $V_{\iF,\iv}$,
hence we add an edge leading to such a neighbour to the set $E_0$.
In this manner we connect all the vertices $\cG \cup \cP$ to the root by an additional cost of $a_3 \cdot N^2$.

Next once again for each group of variables $F_\iF$ consider the sequence $S \in \{1,2,3\}^\groupg$ which corresponds
to the restriction of the assignment $\phi$ to the variables of $F_\iF$.
For each group gadget $\groupg_\iF^\iB$ for $1 \le \iB \le a_1$ 
and for each sequence $S_0 \in \{1,2,3\}^\blocksize$ such that $S_0 \not= S$ we add to $E_0$ one edge 
connecting $x_{S_0}$ with a vertex of a set $V_{\iF,\iv}$ for some $\iv$
since we know that at least one such vertex exists.
Unfortunatelly for the vertex $x_S$ we can not do the same because 
this vertex does not have a neighbour in any set $V_{\iF,\iv}$
hence we add to the set $E_0$ two edges $x_Sx_S'$ and $x_S'r$.
In this way for each group gadget we add to the set $E_0$ edges of total weight $3^\blocksize \cdot N^3+1$,
summing over all the group gadgets this gives $a_2 \cdot N^3 + a_6$.

The only terminals that are not connected to the root by edges of the set $E_0$ are vertices corresponding to clauses of the formula $\Phi$.
For each vertex $c_\iC^{\ib}$ we pick any group of variables $F_\iF$ that satisfies that clause
and add to the set $E_0$ the edge $x_S'c_\iC^{\ib}$ where $S$ is the sequence devoted the assignment of the variables $F_\iF$.
Observe that $x_S'$ is already reachable from the root by edges from the set $E_0$.
Since the cost of each such edge is $N^4$ we use additional cost of $a_1 \cdot N^4$ and have the set $E_0$ spanning all the terminals.

Since the sum of weights of the edges of the set $E_0$ equals to $\goalsize = a_1 \cdot N^4 + a_2 \cdot N^3 + a_3 \cdot N_2 + a_4 \cdot N + a_5 + a_6$
the lemma follows.
\end{proof}

\begin{lemma}\label{lem:lowerst2}
If there exists a tree in the graph $G$ spanning all terminals with the sum of weights of edges not exceeding $\goalsize$,
then $\Phi$ has a satisfying assignment.
\end{lemma}

\begin{proof}
Let $G_0=(V_0,E_0)$ be a minimum weight tree spanning all the terminals in $G$.
Firstly we show that $V_0$ contains two vertices out of each three $v_{\iv}^1,v_{\iv}^2,v_{\iv}^3$
and also contains exactly one vertex $x_S'$ out of each group gadget.
Later we show that for each $1 \le \iF \le n'$ 
the set of sequences $S$ indexing vertices $x_S' \in V_0$ for group gadgets $B_\iF^\iB$ for $1 \le \iB \le a_1$
contains only a few distinct elements.
This will be enough to show a satisfying assignment.

Let us recall that by $N$ we denote the number of vertices in $G$.
Observe that $a_1+a_2+a_3+a_4+a_5+a_6 < N$ since in the previous lemma we have constructed a tree containing exactly that many edges.
Because of this inequality we have $(a_1+1) \cdot N^4 > \goalsize$, hence we infer that in the set $E_0$ there are at most $a_1$ edges
of weight $N^4$. 
Observe that for each terminal vertex $c_\iC^{\ib}$ for $1 \le \iC \le m$, $0 \le \ib \le 5\blocksize n'$
all the incident edges in the graph $G$ are of weight exactly $N^4$ and moreover there are no
edges connecting two terminals.
Since there are $a_1$ vertices $c_\iC^\ib$ we know that the set $E_0$ contains exactly $a_1$
edges of weight $N^4$ and all the vertices $c_\iC^{\ib}$ are leaves in the tree $G_0$.

Now we focus on terminal vertices $x_S$.
In each group gadget there are exactly $3^\blocksize$ such vertices which gives $a_2$ vertices in the whole graph $G$.
As vertices $c_\iC^{\ib}$ are leaves in the tree $G_0$
for each vertex $x_S$ the set $E_0$ either contains the edge $rx_S'$ of weight $N^3$ or one of the edges 
of weight $N^3$ incident with $x_S$.
Consequently the set $E_0$ contains at least $a_2$ edges of weight $N^3$ which means that it contains exactly
$a_2$ edges of weight $N^3$ because $a_1 \cdot N^4 + (a_2+1) \cdot N^3 > \goalsize$.

Using similar argument we show that the set $E_0$ contains at least $a_3$ edges of weight $N^2$,
since each terminal from the set $\cG \cup \cP$ needs to have an incident edge in $E_0$, $|\cG \cup \cP| = a_3$
and the mentioned vertices form an independent set.
Consequently the set $E_0$ contains exactly $a_3$ edges of weight $N^2$ because 
$a_1 \cdot N^4 + a_2 \cdot N^3 + (a_3+1) \cdot N^2 > \goalsize$
and all the vertices $\cG \cup \cP$ are leaves in the tree $G_0$.

As a consequence of all the above arguments we infer that for each vertex $v_\iv^\ivup \in V_0$ 
the simple path between $v_\iv^\ivup$ and $r$ in the tree $G_0$ contains one of the incident to $v_\iv^\ivup$
edges of weight $N$. This edge connects $v_\iv^\ivup$ directly to the root or to some vertex from the set $\cH \cup \cQ \cup \cW$.
Since all guards $\cG$ are terminals we know that the set $V_0$ contains at least two out of each three vertices $v_{\iv}^1,v_{\iv}^2,v_{\iv}^3$
for any $\iv \le \blocksize$ in each group gadget.
Hence the set $V_0$ contains at least $a_4$ vertices $v_\iv^\ivup$.
Since for each vertex $v_\iv^\ivup \in V_0$ we need to have an edge incident to it of weight $N$ in the set $E_0$ and 
$$a_1 \cdot N^4 + a_2 \cdot N^3 + a_3 \cdot N^2 + (a_4+1) \cdot N > \goalsize$$
we prove that there are exactly $a_4$ vertices $v_\iv^\ivup$ in the set $V_0$.
In particular, this implies that out of each triple $(v_\iv^1,v_\iv^2,v_\iv^3)$ from any group gadget the set $V_0$ contains exactly two vertices.

Moreover, since we have only $a_4$ edges of weight $N$ in $E_0$,
for each vertex $v_\iv^\ivup \in V_0$ exactly one incident edge of weight $N$ is in $E_0$.
This implies that for each vertex $v_\iv^\ivup \in V_0$ the simple path between $v_\iv^\ivup$ and $r$ in the tree $G_0$
consists of one edge of weight $N$ or two edges incident to some vertex from $\cH \cup \cQ \cup \cW$, one of weight $N$ and one of weight $1$.

Since out of each triple $(v_\iv^1,v_\iv^2,v_\iv^3)$ from any group gadget the set $V_0$ contains exactly two vertices
in each group gadget $\groupg$, the vertex $x_S$, where $S$ is such a sequence that satisfies $V_\groupg \setminus S(V_\groupg) = V_0 \cap V_\groupg$,
has to be connected to the root through edges $x_Sx_S'$ and $x_S'r$.
Since there are $n'a_1 = a_6$ group gadgets the set $E_0$ contains at least $a_6$ edges $x_Sx_S'$.

Now we prove an upper bound on the number of edges of weight $1$ in the set $E_0$ that are incident with the root.
Since all the previous lower bounds are applied to disjoint sets of edges and the sum of weights of edges in $E_0$ 
is not greater than $\goalsize$ then in the set $E_0$ there are at most $\goalsize-(a_1 \cdot N^4 + a_2 \cdot N^3 + a_3 \cdot N^2 + a_4 \cdot N + a_6) = a_5$
edges incident with the root of weight $1$.

Consider any $\iF,\iv$ such that $1 \le \iF \le n'$, $1 \le \iv \le \blocksize$.
By $L_{\iF,\iv}$ let us denote the sequence containing vertices $v \in V_{\groupg_\iF^\iB,\iv}$ from all the group gadgets $\groupg_\iF^\iB$ for $1 \le \iB \le a_1$.
In the sequence $L_{\iF,\iv}$ vertices $v_{\iv}^\ivup$ are sorted in nondecreasing order of $\iB$ and for the same value of $\iB$ by increasing value of $\ivup$.
Recall that we know that for each vertex $v_{\iv}^\ivup \in V_0$ of the group gadget $\groupg_\iF^\iB$
the simple path between $v_{\iv}^\ivup$ and the root $r$ in the tree $G_0$ contains either a single edge
or exactly two edges incident with some vertex of the set $\cH\cup \cQ \cup \cW$.
Moreover, recall that the only vertex from the set $L_{\iF,\iv}$ that is a neighbour of the root $r$ is the vertex $v_{\iv}^1$ from the gadget $B_\iF^1$.
Observe that each edge of weight $1$ connecting a vertex from $\cH \cup \cQ \cup \cW$ with the root $r$
may belong to at most two simple paths in the tree $G_0$ between the root $r$ and some vertex $v_\iv^\ivup \in V_\groupg$
for some group gadget $\groupg$.
Since there are $2a_1$ vertices in the set $V_0 \cap L_{\iF,\iv}$, and only one of them can be connected to the
root $r$ with a single edge, for each $\iF,\iv$
the set $E_0$ contains at least $a_1$ edges connecting $r$ with some vertex  from the set $\cH \cup \cQ \cup \cW$.
Together with the upper bound of $a_5=\blocksize n' a_1$ edges of weight $1$ in the set $E_0$ incident with the root $r$ we
know that for each $\iF,\iv$ the set $E_0$ contains exactly $a_1$ edges connecting $r$
with a vertex from the set $\cH \cup \cQ \cup \cW$ with sub- and superscripts $\iF$ and $\iv$.

For any $\iF \le n',\iv \le \blocksize$ consider a sequence $\ivupseq_{\iF,\iv}=(\ivup_1,\ldots,\ivup_{a_1}) \in \{1,2,3\}^{a_1}$ where $\ivup_\iB=\ivup$  
iff the vertex $v_{\iv}^{\ivup} \in V_{\groupg_\iF^\iB}$ does not belong to the set $V_0$. 
We want to show that for any sequence $\ivupseq_{\iF,\iv}$ almost all its elements have exactly the same value.
Consider a pair $\ivup_\iB,\ivup_{\iB+1} \in \ivupseq_{\iF,\iv}$ such that $\ivup_\iB > \ivup_{\iB+1}$. 
\begin{itemize}
  \item If $\ivup_\iB \le 2$ then obviously $\ivup_\iB = 2$ since $\ivup_\iB > \ivup_{\iB+1} \ge 1$.
  In this case $\ivup_{\iB+1}=1$ and there is a vertex in the sequence $L_{\iF,\iv}$ (namely $v_{\iv}^3 \in V_{\groupg_\iF^\iB}$)
  that belongs to $V_0$ and both its successor and predecessor exist and do not belong to $V_0$.
  \item If $\ivup_\iB = 3$ then $\ivup_{\iB+1}=2$ since otherwise we would have two consecutive
  vertices from $L_{\iF,\iv}$ outside of the set $V_0$ and there would exist a terminal vertex $p_\iv^{\iF,\iB} \in \cP$ 
  that is not spanned by the tree $G_0$.
  In the case $3 = \ivup_\iB > \ivup_{\iB+1} = 2$ we also have a situation 
  where there exists a vertex in the sequence $L_{\iF,\iv}$ that belongs to $V_0$ 
  and both its successor and predecessor exist and do not belong to $V_0$.
\end{itemize}
Since in both cases we have an edge in $E_0$ that is of weight $1$ and is incident with the root
and belongs to exactly one simple path between $r$ and any vertex $v \in V_\groupg$ for any group gadget $\groupg$,
this situation can not happen more than once because otherwise there would be more that $a_5$ edges
in the set $E_0$ that are incident with the root $r$ and are of weight $1$.
Conseqently each sequence $\ivupseq_{\iF,\iv}$ changes at most $5$ times since it can decrease only once
and hence increase at most $4$ times.
Because each sequence $\ivupseq_{\iF,\iv}$ is of length $a_1$ and there are $\blocksize n'$ such sequences
using a pigeon hole principle we infer that 
there exists an integer $\ib \in [0,5\blocksize n']$ such that for each $1 \le \iF \le n'$,$1 \le \iv \le \blocksize$,$1 \le \iC \le m$ 
we have $\ivup_{\ib m + 1}=\ivup_{\ib m + \iC}$ where $\ivup_{\ib m + 1},\ivup_{\ib m + \iC} \in \ivupseq_{\iF,\iv}$.

We create an assignment $\phi$ that satisfies $\Phi$. For a group of variables $F_\iF$ we take an assignment corresponding
to the sequence obtained by taking the $(\ib m+1)$-th element of sequences $\ivupseq_{\iF,\iv}$ for $1 \le \iv \le \blocksize$.
Now we prove that $\phi$ satisfies all the clauses of the formula $\Phi$ and hence is a satisfying assignment.
Consider a clause $C_\iC$ of the formula $\Phi$.
Let us focus on the vertex $c_\iC^\ib$. 
Since it is a terminal it has an incident edge in the set $E_0$ and we know that there is exactly one such edge.
Let $x_S'$ be the second end-point of this edge and let $\iF$ be such an index that $x_S'$ belongs 
to the group gadget $B_\iF^{\ib m + \iC}$.
Since in the graph $G$ the vertex $c_\iC^\ib$ is only adjacent to vertices $x_S'$ such that the sequence $S$
corresponds to a satisfying assignment of the group of variables $F_\iF$ we know that $\phi$ satisfies the clause $C_\iC$
and in general the whole formula $\Phi$.
\end{proof}

\paragraph{Pathwidth bound}

\begin{lemma}\label{lem:lowerst3}
Pathwidth of the graph $G$ is at most $\blocksize n'+O(3^\blocksize)$.
Moreover a path decomposition of such width can found in polynomial time.
\end{lemma}

\begin{proof}
We give a mixed search strategy to clean the graph with $\blocksize n'+O(3^\blocksize)$ searchers.
First we put a searcher in the root $r$ and this searcher remains there till the end of the cleaning process.
For a gadget $\groupg$ we call the vertices $v_{\iv}^1$ and $v_{\iv}^3$, $1 \le \iv \le \blocksize$, as {\em entry vertices} and {\em exit vertices}
respectively.
We search the graph in $a_1 = \numcopies$ rounds.
In the beginning of round $\iB$ there are searchers on the entry vertices of the gadget $\groupg_\iF^\iB$ for every $\iF \le n'$.
Let $1 \le \iC \le m$ and $0 \le \ib < 5\blocksize n'$ be integers such that $\iB = \iC + m\ib$.
We place a searcher on $c_\iC^\ib$.
Then, for each $1 \le \iF \le n'$ in turn we:
\begin{itemize}
  \item put $O(3^\blocksize)$ searchers on all vertices of the group gadget $B_\iF^\iB$,
  \item put $2\blocksize$  searchers on all $2\blocksize$ vertices $p \in \cP$, $q \in \cQ$ that are adjacent to some vertex $v_\iv^\ivup$ in the group gadget $\groupg_\iF^\iB$,
  \item put $\blocksize$ searchers on the entry vertices of the group gadget $B_\iF^{\iB+1}$ (in round $a_1$ we put $\blocksize$ searchers
      on vertices $w_{\iF,\iv}$ for $1 \le \iv \le \blocksize$),
  \item remove searchers from all vertices of the group gadget $B_\iF^\iB$,
  \item remove $2\blocksize$ searchers from vertices from the set $\cP \cup \cQ$.
\end{itemize}
The last step of the round is removing a searcher from the vertex $c_\iC^\ib$.
After $a_1$ rounds the whole graph $G$ is cleaned.
Since we reuse $O(3^\blocksize)$ searchers for cleaning group gadgets $\blocksize n'+O(3^\blocksize)$ searchers suffice to clean the graph.

Using the above graph cleaning process a path decomposition of width $\blocksize n'+O(3^\blocksize)$ can be constructed in polynomial time.
\end{proof}

We are now ready to conclude the proof of Theorem \ref{thm:wst-lower}.
Suppose \weightedst can be solved in $(3-\eps)^p |V|^{O(1)}$ for graphs with weights bounded by $|V|^4$ provided that we are given a path decomposition of width $p$.
Let $\lambda = \log_3(3-\eps) < 1$.
We choose $\blocksize$ large enough such that $\frac{\log 3^\blocksize}{\lfloor \log 3^\blocksize \rfloor} < \frac{1}{\lambda}$.
Given an instance of SAT we construct an instance of \weightedst using the above construction and the chosen value of $\blocksize$.
Next we solve \weightedst using the $3^{\lambda p} |V|^{O(1)}$ time algorithm.
Lemmas~\ref{lem:lowerst1},\ref{lem:lowerst2} ensure correctness, whereas Lemma~\ref{lem:lowerst3} implies that running time of our algorithm is $3^{\lambda \blocksize n'} |V|^{O(1)}$,
however we have $3^{\lambda \blocksize n'}=2^{\lambda \blocksize n'\log 3}=2^{\lambda n'\log 3^\blocksize}=2^{\lambda n \log 3^\blocksize / \lfloor \log 3^\blocksize \rfloor } = 2^{\lambda' n}$ for some $\lambda' < 1$. This concludes the proof.
\qed

It remains to show a reduction from the weighted to the unweighted case.
Since all the weights are positive integers upper bounded by $|V|^4$ (which is a polynomial) for an edge $e$ 
of weight $c(e)$ we can subdividide it $c(e)-1$ times obtaining an unweighted version of the problem.
Observe that in the \weightedst problem we were minimizing the weight of edges and in the \steinertree problem
we are minimizing the number of nodes, but for the unweighted graph minimizing the number of edges
is the same as minimizing the number of Steiner nodes.
The last thing to show is that after several subdivision operations the pathwidth of the graph does not increase significantly.

\begin{lemma}
Let $G'$ be a graph obtained from $G=(V,E)$ by subdividing each edge $e \in E$ $c(e)-1$ times.
Given a path decomposition of $G$ of width $p$ one can in polynomial time construct a path decomposition of $G'$ of width at most $p+2$.
\end{lemma}

\begin{proof}
Assume we are given a path decomposition of $G$ of width $p$. 
Let $e=uv$ be an arbitrary edge in $G$ with $c(e) > 1$.
By $\bag{e}$ let us denote any fixed bag that covers $e$, i.e., contains both $u$ and $v$.
Let $\{x_{e,1},\ldots,x_{e,c(e)-1}\}$ be vertices added to the graph after subdividing the edge $e$ $c(e)-1$ times.
Construct bags $\bag{e,0} = \bag{e} \cup \{x_{e,1}\}$ and $\bag{e,i} =  \bag{e} \cup \{x_{e,i}, x_{e,i+1}\}$ for $i=1,\ldots,c(e)-2$.
Insert bags $\bag{e,i}$ for $i=0,\ldots,c(e)-2$ in this order after the bag $\bag{e}$ in the given path decomposition.
If $\bag{e}$ is the fixed bag for many edges $e$, insert the newly created sequences of bags in an arbitrary order after $\bag{e}$.
It is easy to see that after adding additional bags $\bag{e,i}$ for all edges the width of the path decomposition increases by at most $2$
and the new path decomposition is a proper path decomposition of the new graph.
\end{proof}

We can now conclude this section with the following theorem.

\begin{theorem}\label{thm:st-lower}
Assuming SETH, there cannot exist a constant $\eps > 0$ and an algorithm that given an instance $(G=(V,E), T)$ together with a path decomposition of the graph $G$ of width $p$ solves the \steinertree problem in $(3-\eps)^p |V|^{O(1)}$ time.
\end{theorem}


==> pathwidth.tex <==
\section{Improving time complexity when parameterized by pathwidth}

For problems where we choose a subset of edges there is no need to remember the side of the cut 
for the vertex which has no incident edge yet chosen.
This could cause problems for join bags when parameterized by treewidth, however for problems parameterized by pathwidth
there is no such problem because there are no join bags.

This immediately gives an improvement of the time complexity for the following problems:
\begin{itemize}
  \item k-Leaf Spanning Tree, from $6^t$ to $5^{pw}$,
  \item k-Leaf Outbranching, from $8^t$ to $7^{pw}$,
  \item full degree spanning tree, from $4^t$ to $3^{pw}$,
  \item directed longest cycle, from $8^t$ to $7^{pw}$,
  \item directed cycle cover, from $8^t$ to $7^{pw}$.
\end{itemize}

for problems when we remember the parity of the degree of each vertex
this observation needs some adjustment in the local object definition, and we get:

\begin{itemize}
  \item graph metric tsp, from $4^t$ to $3^{pw}$,
  \item longest cycle, from $4^t$ to $3^{pw}$.
\end{itemize}


==> reversing-cycles.tex <==
\section{Improving time complexity of undirected problems}

We avoid using cuts and use the trick also used by Bj{\"o}rklund and Bj{\"o}rklund et al.
We show that using the trick with reversing undirected cycle we can prove faster algorithms for $k$-leaf spanning tree
and obtain alternative solutions (without cut\&count) with the same time complexity as with cut\&count for the following problems:
FVS, Undirected Longest Cycle.

\subsection{k-Leaf Spanning Tree}

We are interested in a subset of $n-1$ directed edges. Opposite edges have the same variable.
Each vertex can have at most one incoming edge.
the root has no incoming edges.

State: we store the number of incoming edges $\{0, 1\}$ and the number of outgoing edges $\{0, 1+\}$.

Objects corresponding to proper $k$-leaf arborescences will be counted once, whereas 
objects which are not connected will be counted twice, because we can reverse all the cycles (they are disjoint)
and get the same monomial.

The number of states $4^t$, merging using FSC.

\subsection{FVS}

Described by Onufry in emails.

\subsection{Longest Path/Cycle}

Described in a separate file hamilton.tex.


